Design Automation for Obfuscated Circuits with Multiple Viable Functions

Gate camouflaging is a technique for obfuscating the function of a circuit against reverse engineering attacks. However, if an adversary has pre-existing knowledge about the set of functions that are viable for an application, random camouflaging of gates will not obfuscate the function well. In this case, the adversary can target their search, and only needs to decide whether each of the viable functions could be implemented by the circuit. In this work, we propose a method for using camouflaged cells to obfuscate a design that has a known set of viable functions. The circuit produced by this method ensures that an adversary will not be able to rule out any viable functions unless she is able to uncover the gate functions of the camouflaged cells. Our method comprises iterated synthesis within an overall optimization loop to combine the viable functions, followed by technology mapping to deploy camouflaged cells while maintaining the plausibility of all viable functions. We evaluate our technique on cryptographic S-box functions and show that, relative to a baseline approach, it achieves up to 38\% area reduction in PRESENT-style S-Boxes and 48\% in DES S-boxes.

==> related_work.tex <==
Over the last few years, there have been several proposals for look-alike cells in which it is difficult for the adversary to infer the gate function from its appearance~\cite{cocchi-14}. For example, works have proposed to do this using oxide-terminated vias~\cite{chow-2007-integrated,rajendran-13}, using different threshold voltages~\cite{iyengar-15,collantes-16}, or using doping to create stuck-at-faults~\cite{becker-13}. The attacker model in these works allow that the adversary can identify the obfuscated cells by optical inspection during reverse engineering, but do not allow her to observe the particular aspect of each cell instance that determines its functionality.

When gate camouflaging technologies are deployed in a circuit, the uncertainty about the functions of gate instances leads to a number of plausible functions for the overall circuit that is exponential in the number of camouflaged gates. In the scenario where intermediate values can be read out of registers through a scan chain, SAT-based attacks~\cite{elmassad-15} and defenses~\cite{yasin2016sarlock,xie2016mitigatingsat} are applicable. To protect against reverse engineering by querying the circuit, intermediate values should be inaccessible~\cite{yasin-15}, especially in a security-critical design. This mitigates the threat of SAT attacks. 

Although SAT-based attacks can be prevented by making circuit values inaccessible, a circuit function can be reverse engineered without observable values when some information is known about its function. For example, an attacker can check whether the plausible functions contain a particular function of interest (e.g. a viable function) by checking satisfiability of a QBF problem that is similar to equivalence checking, but with unconstrained side inputs that select which of the plausible functions is realized by the circuit~\cite{subramanyan-14}.
%Because the unconstrained side inputs can choose any plausible function, the result of this check indicates either that the viable function is in the set of plausibly implemented functions, or that the viable function is not plausible and can be ruled out.
Note that the attacker is able to perform this check {\itshape without being able to observe or control any values in the circuit}. This attack can be prevented if the viable functions of the circuit are a subset of the plausible functions of the circuit.
%If this condition is met, then an attacker checking whether a viable function is plausible will always find that it is, and thus learn nothing about which viable function is actually implemented. 

In another context outside of security, there has been work that considers the problem of creating polymorphic circuits that implement two different functions, depending on the operating conditions such as supply voltage or temperature. One such work uses Cartesian Genetic Programming (CGP) to evolve polymorphic circuits~\cite{gajda2009gate}, and later work proposes to speed up the fitness function evaluation of CGP with SAT-based equivalence checking~\cite{sekanina2012sat}. These techniques, while promising, do not appear to be scalable as the number of functions grow, and may not converge to a solution even when the number of polymorphic functions is small. Avoiding the daunting task of trying to evolve a circuit that plausibly implements up to 16 different functions, we rely in this work on an algorithmic synthesis-based approach that is guaranteed to produce a solution. 


